Automatic Song Translation for Tonal Languages

This paper develops automatic song translation (AST) for tonal languages and addresses the unique challenge of aligning words' tones with melody of a song in addition to conveying the original meaning. We propose three criteria for effective AST -- preserving meaning, singability and intelligibility -- and design metrics for these criteria. We develop a new benchmark for English--Mandarin song translation and develop an unsupervised AST system, Guided AliGnment for Automatic Song Translation (GagaST), which combines pre-training with three decoding constraints. Both automatic and human evaluations show GagaST successfully balances semantics and singability.

==> 2022_acl_song_translation/sections/5-experiments.tex <==
\section{Experiments}

\subsection{Training Datasets and Model Configuration}
\label{sec:dataset}
\textbf{WMT translation data.} We use the news commentary and back-translated news datatsets from WMT14, which consisting of about 29.6 million en2zh sentence pairs.  \\
\textbf{Monolingual lyrics data.} We collect monolingual lyrics in both Mandarin and English from the web, which contains about 12.4 million lines of lyrics for Mandarin and 109.5 million for English after removing the duplication.\\
\textbf{Lyrics translation data.} We crawl a small set of lyrics translation data from the web,\footnote{https://lyricstranslate.com/} which contains 140 thousands pairs of English-to-Mandarin lines. The translations are not singable.

We preprocess all data with fastBPE~\citep{sennrich-etal-2016-neural} and a code size of 50,000. We choose standard encoder-decoder Transformer~\citep{vaswani2017attention} model with an architecture of 768 hidden units, 12 heads, GELUactivation, a dropout rate of 0.1, 512 max input length, 12 layers in encoder, 12 layers in decoder.


% \subsection{Model Configuration}
% We choose standard encoder-decoder Transformer~\citep{vaswani2017attention} model with an architecture of 768 hidden units, 12 heads, GELUactivation, a dropout rate of 0.1, 512 max input length, 12 layers in encoder, 12 layers in decoder.

\subsection{Evaluation Dataset}
\label{sec:eval_data}
For evaluation, we need aligned triples (melody $M$, source lyrics $X$, target reference lyrics $Y$), where $M$ and $X$ are syllable-to-notes aligned; and the reference $Y$ should be singable and intelligible. Without copyright and accessibility to the singable translated songs, we chose fifty songs from the lyrics translation dataset that have open-source music sheets on the web, and create aligned triples manually. However, the reference lyrics in this dataset do not necessarily resemble song-text style and are not singable, we use them merely to provide a coarse estimation for semantic changes. 
Twenty songs are used as the valid set (464 lines) and thirty songs as the test set (713 lines).


\subsection{Evaluation Metrics}
\label{sec:eval_metrics}
To evaluate the ability of given \abr{ast} system in preserving semantics, singability and intelligibility, we design both objective and subjective evaluations.

\begin{table*}[t]
  \small
	\centering
	\resizebox{\linewidth}{!}{
	\begin{tabular}{clcccccc}
		\toprule
		 Syllable-notes & \multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{Pitch} & \multicolumn{1}{c}{Rhythm} & \multicolumn{2}{c}{Length} & Semantics\\
		 Assignment & & contour~$\uparrow$ & shape~$\uparrow$ & avg \# of missed rests~$\downarrow$ & longer~$\downarrow$ &  shorter~$\downarrow$ & BLEU~$\uparrow$ \\
		\midrule
% 		\midrule
		 \multirow{4}{*}{one-to-one} & \name{} w/o constraints & 0.27 & - & 0.53 & 9 (0.09) & 0 & 24.0 \\ % 0 0 0
		 & \name{} & 0.52 & - & 0.31 & 26 (0.21) & 0 & 16.9  \\  % 0.5 0 1.5
		 & \ \ --only contour & 0.52 & - & 0.45 & 26 (0.21) & 0 & 16.8  \\ % 0.5 0 0
		 & \ \ --only rest & 0.27 & - & 0.31 & 11 (0.11) & 0 & 23.8  \\ % 0 0 1.5
        \midrule
        \multirow{5}{*}{one-to-many} & \name{} w/o constraints & 0.26 & 0.50 & 0.56 & 4 (0.11) & 0 &  22.1  \\
		 & \name{} & 0.47 & 0.57 & 0.29 & 13 (0.14) & 0 & 15.9  \\
		 & \ \ --only contour & 0.48 & 0.51 & 0.44 & 7 (0.12) & 0 & 15.8 \\
		 & \ \ --only shape & 0.26 & 0.57 & 0.51 & 4 (0.11) & 0 & 21.6  \\
		 & \ \ --only rest & 0.26 & 0.50 & 0.31 & 5 (0.11) & 0 & 21.6  \\
        \bottomrule
	\end{tabular}
	}

	\caption{Objective results on test set of \name{} with different constraints under one-to-one and one-to-many assignments. All results here use the same pretraining checkpoint and length tags are applied. For length score, 9 (0.09) means that 9 out of 713 samples are longer than the predefined length with an average ratio 0.09. }
	\label{tab:main_res} 
\end{table*}

\begin{figure*}[t]
	\centering
	\begin{subfigure}[h]{0.32\textwidth}
	    \captionsetup{justification=centering}
		\centering
		\includegraphics[width=\textwidth, trim={0.2cm 0.2cm 0.1cm 0.1cm}, clip=true]{2022_acl_song_translation/figures/constraint_contour_big.pdf}
		\caption{Different contour constraints.}
		\label{fig:constraint_contour}
	\end{subfigure}
	\begin{subfigure}[h]{0.32\textwidth}
	    \captionsetup{justification=centering}
		\centering
		\includegraphics[width=\textwidth, trim={0.2cm 0.2cm 0.1cm 0.1cm}, clip=true]{2022_acl_song_translation/figures/constraint_shape_bleu_big.pdf}
		\caption{Different shape constraints.}
		\label{fig:constraint_shape}
	\end{subfigure}
	\begin{subfigure}[h]{0.32\textwidth}
	    \captionsetup{justification=centering}
		\centering
		\includegraphics[width=\textwidth, trim={0.2cm 0.2cm 0.1cm 0.1cm}, clip=true]{2022_acl_song_translation/figures/constraint_rest_punc_big.pdf}
		\caption{Different rest constraints.}
		\label{fig:constraint_rest}
	\end{subfigure}

	\caption{Trade-off between semantics and lyric-music alignments; all curves are drawn for the valid set.}
	\label{fig:ablation_constraints}
\end{figure*}

\subsubsection{Objective Evaluation}

For \textbf{semantics}, we follow the common practice and calculate the BLEU scores~\citep{papineni2002bleu} between the translated lyrics and corresponding reference. For singability and intelligibility, we use the following metrics:

For \textbf{length alignment}, we computes: 1) $N_l$, the number of samples that has length longer than the predefined length $L_i$; 2) $N_s$, that are shorter than $L_i$. And for each case, we show the average error ratio of $\{\Delta l_i / L_i\}_1^{N_{[\cdot]}}$.

For the three scores for \textbf{pitch} and \textbf{rhythm alignment}, we normalize the score to 0 -- 1.0 by the length of alignment pairs $L_i$, that is, based on Equation~\ref{eq:shape_score},\ref{eq:contour_score} and \ref{eq:rest_constraint},
\begin{equation}
    s_{[\cdot]} = \sum_1^{L_i}S_{[\cdot]}^i/L_i,
\end{equation}


\subsubsection{Subjective Evaluation}
To demonstrate whether the proposed metrics align with actual human experiences and examine the quality of the translated songs by \name{}, we conduct human evaluations. We randomly select five songs from the test set and show the music sheets\footnote{Without singing voice synthesize tools, following \citet{sheng2020songmass}, we show the annotators the music sheets without singing} of the first ten sentences of each translated song by \name{} to five annotators from Music School. 

Following mean opinion score (MOS)~\citep{rec1994p} in speech synthesize task, we use five-point scales (1 for bad and 5 for excellent) in four aspects: 1)~\textit{sense}, fidelity to the meaning of the source lyric; 2)~\textit{style}, whether the translated lyric resembles song-text style; 3)~\textit{listenability}, whether the translated lyric sounds melodious with the given melody; 4)~\textit{intelligibility}, whether the audience can easily comprehend the translated lyrics if sung with provided melody. The latter two qualities require the annotators to sing the song themselves.


\subsection{Hyper-parameters and Trade-offs}
\label{sec:tradeoff}
\name{} adds constraints in the decoding scoring functions to enforce lyric-music alignments. There are trade-offs between semantics and other alignments. We analyze the increasing curves of pitch alignment scores against BLEU on valid set, and chose the hyperparameters where the alignment scores increase fast while the BLEU decrease slow. The \textit{REST} constraint does not affect the BLEU~(Table~\ref{tab:main_res}) but the number of punctuation. We should prevent a large increase in the number of punctuation while reducing the mismatches between the \textit{REST} and semantic segmentation. Based on Figure~\ref{fig:ablation_constraints}, we chose: $\lambda_{pc}=0.5;\ \lambda_{ns}=1.5;\ \lambda_{R}=3.0$.

\subsection{Evaluation Results}
\label{sec:results}
\subsubsection{Objective Evaluation Results}

Table~\ref{tab:main_res} compares the performance of \name{} with different constraints. As described in Section~\ref{sec:gagast}, we predefine the note(s) groups and use two syllable-notes assignments: one-to-one and one-to-many. From results in Table~\ref{tab:main_res}, we can see,

\begin{itemize}
    \item The proposed length tag [LEN\$i] helps to produce lyrics that fit into the predefined note(s) groups. In all cases, less than 30 out of 713 lines produces a longer sentence with ratio less than 0.22; and no short cases.
    \item We use the \name{} w/o constraints except for length tags as our baseline. Compared to which, \name{} with full constraints is able to increase both pitch and rhythm alignments significantly with a fairly slow drop in BLEU\footnote{For references, we found three officially translated Disney songs in Mandarin and computes the BLEU among the human translated singable lyrics with the lyrics translation from our dataset, the average BLEU is only 12.3.}. It almost doubles the pitch contour alignment score, which affect the intelligibility the most. 
    \item Each constraint applied is able to increase the corresponding alignment performance.
\end{itemize}

\subsubsection{Subjective Evaluation Results}

To examine if the proposed constraints are able to improve the singability and intelligibility, and to evaluate the quality of translated songs by \name{}, we conduct subjective evaluation and compare the \name{} w/o constraints to fully constrained \name{} in Table~\ref{tab:subjective}. We compute the confidence intervals for all aspects. Results show that,

\begin{itemize*}
    \item The proposed constraints is able to significantly improve the intelligibility for audience. 
    \item The proposed constraints is able to improve the listening experiences for human with minor significance. The listenability for audience reflects the singability for performer.
    \item Add constraints do cause a trade-off between the semantics (sense) and other qualities. 
    \item Overall, the annotators are satisfy with the translated songs by the proposed baseline \name{}. All aspects receive an average score around 3.5 out of 5. 
\end{itemize*}

The subjective evaluation demonstrates that the proposed alignments, constraints and the acceptable notes transitions for Mandarin~(Figure~\ref{fig:tone_contour}) are reasonable. They are able to improve the singability and intelligibility. Although there's a trade-off, due to the lack of singing voice synthesize tools, the subjective evaluation is actually in favor the sense/style evaluation compared to listenability/intelligibility.

We add case studies and post three translated songs by \name{} sung by ourselves on demo page \href{https://gagast.github.io/posts/gagast}{https://gagast.github.io/posts/gagast}.

\begin{table}[t]
  \small
	\centering
	\resizebox{\linewidth}{!}{
	\begin{tabular}{cccccc}
		\toprule
		 Model & Song & \textit{sense} & \textit{style} & \textit{listenability} & \textit{intelligibility} \\
		\midrule
% 		\midrule
		 \multirow{3}{*}{} & Song1 & 3.4 & 3.0 & 3.2 & 3.4 \\
		 & Song2 & 3.6 & 3.9 & 3.5 & 3.8 \\
		 \name{} & Song3 & 3.7 & 3.6 & 3.4 & 3.5 \\
		 w/o constraints & Song4 & 3.2 & 3.0 & 2.8 & 3.0 \\
		 \multirow{2}{*}{} & Song5 & 3.7 & 3.6 & 3.4 & 3.8 \\ 
		 \cmidrule{2-6}
		 & \textbf{Average} & \textbf{3.5} ±0.14 & 3.4 ±0.14 & 3.2 ±0.12 & 3.5 ±0.13 \\
        \midrule{}
        \multirow{6}{*}{\name{}} & Song1 & 3.5 & 3.1 & 3.3 & 3.5 \\
		 & Song2 & 3.4 & 3.7 & 3.5 & 4.0 \\
		 & Song3 & 3.2 & 3.6 & 3.3 & 3.6 \\
		 & Song4 & 2.9 & 3.0 & 3.1 & 3.5 \\
		 & Song5 & 3.4 & 3.6 & 3.2 & 3.9 \\ 
		 \cmidrule{2-6}
		 & \textbf{Average} & 3.3 ±0.15 & 3.4 ±0.15 & \textbf{3.3} ± 0.12 & \textbf{3.7} ±0.13 \\
        \bottomrule
	\end{tabular}
	}
	\caption{Subjective evaluation results for \name{} w/o constraints and \name{}.}

	\label{tab:subjective} 
\end{table}

% \begin{wraptable}{r}{0.5\textwidth}
% 	\centering
% 	\begin{tabular}{l|cc}
% 	\toprule
% 	Metric & Baseline & \name{} \\
% 	\midrule
% 	\textit{sense} & & \\
% 	\textit{xx} & & \\
% 	\textit{listenability} & & \\
% 	\textit{intelligibility} & & \\
% 	\bottomrule
% 	\end{tabular}
% 	\caption{Subjective evaluation results of baseline and \name{}, with 95\% confidence intervals.}
% 	\label{tab:ablation_pretrain} 
% \end{wraptable}

% \subsection{Ablation Studies}

% \subsection{Analyses}
% We conduct more experimental analyses to further explore our \name{} and show how we choose the hyperparameters, i.e, the weights for each constraint. More analyses are listed in the supplementary material, including the effectiveness of length tag and case studies with translated lyrics under different constraints.

% \subsubsection{Pretraining Data}
% \name{} has three kinds of pretraining data: general translation data (denoted as general), monolingual lyrics data (denoted as mono) and lyrics translation data. In order to explore the improvement brought by each part of data, we conduct ablation studies and list the results in Table~\ref{tab:ablation_pretrain}. As we can see, when removing monolingual lyrics data in pretraining stage, the BLEU score drops slightly and the \#longer increases, which demonstrates that monolingual lyrics data can bring knowledge of lyrics domain into the translation model so that improve the model performance. When continue removing the general translation data, the BLEU score further decreases, and the \#longer and \#shorter are dramatically large, which indicates that the pretrained model requires more data to learn the control of length with length tag.
% \begin{table}[!thb]
%   \small
% 	\centering
% 	\resizebox{\linewidth}{!}{
% 	\begin{tabular}{lccccccc}
% 		\toprule
% 		\multirow{2}{*}{Model} & \multicolumn{2}{c}{Pitch} & \multicolumn{1}{c}{Rhythm} & \multicolumn{2}{c}{Length} & \multicolumn{2}{c}{Semantics}\\
% 		 & contour~$\uparrow$ & shape~$\uparrow$ & avg \# of missed rests~$\downarrow$ & \# of longer~$\downarrow$ & \# of shorter~$\downarrow$ & BLEU~$\uparrow$ & Bert-score~$\uparrow$ \\
% 		\midrule
% 		 \name{} & 0.47 & 0.57 & 0.29 & 13 & 0 & 15.9 & 0.81 \\
% 		 \ \ --mono & 0.47 & 0.56 & 0.28 & 49 & 1 & 14.4 & 0.81 \\
% % 		 \ \ --lyrics translation & 0.49 & 0.5 & 0.39 & 14 & 0 & 12.2 & 0.79\\
% 		 \ \ --general \& mono & 0.46 & 0.51 & 0.26 & 150 & 182 & 12.2 & 0.79 \\
%         \bottomrule
% 	\end{tabular}
% 	}
% 	\vspace{0.3cm}
% 	\caption{Pretrain the translation model with different datasets. 713 samples in test set.}
% 	\label{tab:ablation_pretrain} 
% 	\vspace{-0.6cm}
% \end{table}

% \subsubsection{Constraints}
% Adding constraints helps with improving the prosodic alignment, whereas impairs semantic alignment to a certain extent. We conduct a series of experiments with different constraint weights in development set and attempt to trade off between the two alignments according to the results. As shown in Figure~\ref{fig:constraint_contour}, the BLEU score drops and the pitch contour score increase when the weight of pitch contour constraint ($\lambda_{pc}$ in Equation~\ref{eq:all_constraints}) grows larger. It is obvious that when $\lambda_{pc}$ is 0.5, both prosodic and semantic alignments are relatively good, and when $\lambda_{pc}$ rises to 1, the pitch contour score increases a little while the BLEU score drops dramatically. That is why we set $\lambda_{pc}$ to 0.5 in our \name{}.


% We choose 0.5 as the weight of shape constraint ($\lambda_{ns}$ in Equation~\ref{eq:all_constraints}) for the same reason as described in Figure~\ref{fig:constraint_shape}.
% The rest constraint increases the probability of translating [SEP], [punc] or finishing a word when encountering \textit{REST} notes. [SEP] and [punc] will be deleted when calculating the BLEU score, so they have little effect on BLEU score. However, the number of [SEP] and [punc] cannot be too large, otherwise the translated lyrics will be fragmented and do not look like "lyrics".
% For the weight of rest constraint ($\lambda_{rest}$ in Equation~\ref{eq:all_constraints}), we focus on the miss\_rest\_num and the number of [punc] per samples. As can be seen in Figure~\ref{fig:constraint_rest}, when $\lambda_{rest}$ is set to 3, the miss\_rest\_num is relatively low and the number of [punc] is also not too large. According to Figure~\ref{fig:constraint_rest}, we choose 3 as final $\lambda_{rest}$ in our \name{}.


==> 2022_acl_song_translation/sections/7-conclusion.tex <==
\section{Conclusion}

\jbgcomment{Don't just repeat introduction here.  Talk about future work}

This paper introduces a novel task in verse translation -- Automatic Song Translation~(AST) for tonal languages. Compare to prose translation, verse translation is harder as it needs to obey prosody formats in addition to retain the meaning. AST for tonal languages is even more challenge since it needs to align the tones in words with that in music, so that the translated song is singable and intelligible. We introduce three criteria for AST and propose corresponding lyric-music alignment metrics. For this novel task, we propose a baseline AST system GagaST for English-Mandarin song translation and annotate a lyric-music aligned test set to establish benchmark. We design objective and subjective evaluation metrics. Results demonstrate that the proposed lyric-music alignments help to achieve singability and intelligibility and the proposed GagaST is able to translate songs that are melodious and intelligible. 

% Music is an important part of human culture. Song translation helps to break the language barrier so that songs can be performed in different languages and spread worldwide, thereby promoting cultural communications. Unlike traditional translation, it requires the translated lyrics singable with the original melody. We are the first ones to address song translation automatically, and build a benchmark with well-designed evaluation metrics. For singability, linguists and musicians point out that the rhythmic prosody of lyrics and melody should match; and for tonal language such as Chinese, the pitch flow created by tones should align with the melodic contour. However, we lack parallel data to learn such alignments. Therefore, we propose an unsupervised Automatic Song Translation (AST) pipeline, Guided AliGnment for Automatic Song Translation (GagaST), where we pretrain a pure translation model and add melody-guided alignment in the decoding stage during test time. To quantitatively evaluate an AST system, we design a set of objective and subjective evaluation metrics and annotate a music note-syllable aligned test set. Experimental results show that GagaST is able to achieve balance between semantics and singability. Furthermore, the subjective evaluation shows that the translated song also sounds good to humans. 
% \ref{todo}
